Symbol Synchronization for Diffusive Molecular Communication Systems

Symbol synchronization refers to the estimation of the start of a symbol interval and is needed for reliable detection. In this paper, we develop a symbol synchronization framework for molecular communication (MC) systems where we consider some practical challenges which have not been addressed in the literature yet. In particular, we take into account that in MC systems, the transmitter may not be equipped with an internal clock and may not be able to emit molecules with a fixed release frequency. Such restrictions hold for practical nanotransmitters, e.g. modified cells, where the lengths of the symbol intervals may vary due to the inherent randomness in the availability of food and energy for molecule generation, the process for molecule production, and the release process. To address this issue, we propose to employ two types of molecules, one for synchronization and one for data transmission. We derive the optimal maximum likelihood (ML) symbol synchronization scheme as a performance upper bound. Since ML synchronization entails high complexity, we also propose two low-complexity synchronization schemes, namely a peak observation-based scheme and a threshold-trigger scheme, which are suitable for MC systems with limited computational capabilities. Our simulation results reveal the effectiveness of the proposed synchronization~schemes and suggest that the end-to-end performance of MC systems significantly depends on the accuracy of symbol synchronization.

==> Fig/BER_Thr_Fig0/BER_Thr_Fig0.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[cl][cl]{\matlabtextA $\boldsymbol{\xi}_A=[5,14]$}%
\psfrag{010}[cl][cl]{\matlabtextA $\boldsymbol{\xi}_A=[4.5,13]$}%
\psfrag{011}[cl][cl]{\matlabtextA $\boldsymbol{\xi}_A=[4,12]$}%
\psfrag{012}[cl][cl]{\matlabtextA Peak Detector}%
\psfrag{013}[cl][cl]{\matlabtextA Mean Detector}%
\psfrag{014}[bc][bc]{\matlabtextA BER}%
\psfrag{015}[tc][tc]{\matlabtextA Synchronization Threshold, $\xi_B$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $5$}%
\psfrag{001}[ct][ct]{\matlabtextA $10$}%
\psfrag{002}[ct][ct]{\matlabtextA $15$}%
\psfrag{003}[ct][ct]{\matlabtextA $20$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextA $10^{-4}$}%
\psfrag{005}[rc][rc]{\matlabtextA $10^{-3}$}%
\psfrag{006}[rc][rc]{\matlabtextA $10^{-2}$}%
\psfrag{007}[rc][rc]{\matlabtextA $10^{-1}$}%
\psfrag{008}[rc][rc]{\matlabtextA $10^{0}$}%
%
%% </ytick>

==> Fig/BER_Thr_Fig0/Test.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[cl][cl]{\matlabtextA $\boldsymbol{\xi}_A=[5,14]$}%
\psfrag{010}[cl][cl]{\matlabtextA $\boldsymbol{\xi}_A=[4.5,13]$}%
\psfrag{011}[cl][cl]{\matlabtextA $\boldsymbol{\xi}_A=[4,12]$}%
\psfrag{012}[cl][cl]{\matlabtextA Peak Detector}%
\psfrag{013}[cl][cl]{\matlabtextA Mean Detector}%
\psfrag{014}[bc][bc]{\matlabtextA a)}%
\psfrag{015}[bc][bc]{\matlabtextA BER}%
\psfrag{016}[tc][tc]{\matlabtextA Synchronization Threshold, $\xi_B$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $5$}%
\psfrag{001}[ct][ct]{\matlabtextA $10$}%
\psfrag{002}[ct][ct]{\matlabtextA $15$}%
\psfrag{003}[ct][ct]{\matlabtextA $20$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextA $10^{-4}$}%
\psfrag{005}[rc][rc]{\matlabtextA $10^{-3}$}%
\psfrag{006}[rc][rc]{\matlabtextA $10^{-2}$}%
\psfrag{007}[rc][rc]{\matlabtextA $10^{-1}$}%
\psfrag{008}[rc][rc]{\matlabtextA $10^{0}$}%
%
%% </ytick>

==> Fig/BER_Thr_Fig1/BER_Thr_Fig1.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{011}[cl][cl]{\matlabtextA TT Sync.}%
\psfrag{012}[cl][cl]{\matlabtextA PO Sync.}%
\psfrag{013}[cl][cl]{\matlabtextA ML Sync.}%
\psfrag{014}[cl][cl]{\matlabtextA Perfect Sync.}%
\psfrag{015}[cl][cl]{\matlabtextA Peak Detector}%
\psfrag{016}[cl][cl]{\matlabtextA Mean Detector}%
\psfrag{017}[bc][bc]{\matlabtextA BER}%
\psfrag{018}[tc][tc]{\matlabtextA Detection Threshold, $\xi_A$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $0$}%
\psfrag{001}[ct][ct]{\matlabtextA $5$}%
\psfrag{002}[ct][ct]{\matlabtextA $10$}%
\psfrag{003}[ct][ct]{\matlabtextA $15$}%
\psfrag{004}[ct][ct]{\matlabtextA $20$}%
\psfrag{005}[ct][ct]{\matlabtextA $25$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextA $10^{-4}$}%
\psfrag{007}[rc][rc]{\matlabtextA $10^{-3}$}%
\psfrag{008}[rc][rc]{\matlabtextA $10^{-2}$}%
\psfrag{009}[rc][rc]{\matlabtextA $10^{-1}$}%
\psfrag{010}[rc][rc]{\matlabtextA $10^{0}$}%
%
%% </ytick>

==> Fig/BER_Thr_Fig2/BER_Thr_Fig2.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{011}[cl][cl]{\matlabtextA TT Sync.}%
\psfrag{012}[cl][cl]{\matlabtextA PO Sync.}%
\psfrag{013}[cl][cl]{\matlabtextA ML Sync.}%
\psfrag{014}[cl][cl]{\matlabtextA Perfect Sync.}%
\psfrag{015}[cl][cl]{\matlabtextA $\bar{T}^{\mathrm{symb}}=0.5$ ms}%
\psfrag{016}[cl][cl]{\matlabtextA $\bar{T}^{\mathrm{symb}}=1$ ms}%
\psfrag{017}[cl][cl]{\matlabtextA $\bar{T}^{\mathrm{symb}}=2$ ms}%
\psfrag{018}[bc][bc]{\matlabtextA BER}%
\psfrag{019}[tc][tc]{\matlabtextA Detection Threshold, $\xi_A$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $0$}%
\psfrag{001}[ct][ct]{\matlabtextA $5$}%
\psfrag{002}[ct][ct]{\matlabtextA $10$}%
\psfrag{003}[ct][ct]{\matlabtextA $15$}%
\psfrag{004}[ct][ct]{\matlabtextA $20$}%
\psfrag{005}[ct][ct]{\matlabtextA $25$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextA $10^{-4}$}%
\psfrag{007}[rc][rc]{\matlabtextA $10^{-3}$}%
\psfrag{008}[rc][rc]{\matlabtextA $10^{-2}$}%
\psfrag{009}[rc][rc]{\matlabtextA $10^{-1}$}%
\psfrag{010}[rc][rc]{\matlabtextA $10^{0}$}%
%
%% </ytick>

==> Fig/BER_Thr_Fig3/BER_Thr_Fig3.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA Bio Sync.}%
\psfrag{011}[cl][cl]{\matlabtextA Peak Sync.}%
\psfrag{012}[cl][cl]{\matlabtextA ML Sync.}%
\psfrag{013}[cl][cl]{\matlabtextA Ideal Sync.}%
\psfrag{014}[cl][cl]{\matlabtextA $\mathbf{SNR}=[10, 10]$ dB}%
\psfrag{015}[cl][cl]{\matlabtextA $\mathbf{SNR}=[10, 5]$ dB}%
\psfrag{016}[cl][cl]{\matlabtextA $\mathbf{SNR}=[5, 10]$ dB}%
\psfrag{017}[bc][bc]{\matlabtextA BER}%
\psfrag{018}[tc][tc]{\matlabtextA Detection Threshold, $\xi_A$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $0$}%
\psfrag{001}[ct][ct]{\matlabtextA $5$}%
\psfrag{002}[ct][ct]{\matlabtextA $10$}%
\psfrag{003}[ct][ct]{\matlabtextA $15$}%
\psfrag{004}[ct][ct]{\matlabtextA $20$}%
\psfrag{005}[ct][ct]{\matlabtextA $25$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextA $10^{-3}$}%
\psfrag{007}[rc][rc]{\matlabtextA $10^{-2}$}%
\psfrag{008}[rc][rc]{\matlabtextA $10^{-1}$}%
\psfrag{009}[rc][rc]{\matlabtextA $10^{0}$}%
%
%% </ytick>

==> Fig/Concept_Bio/Concept_Bio.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{027}[cl][cl]{\matlabtextA $\hat{t}_s^{\mathtt{thr}}[k]$}%
\psfrag{028}[cl][cl]{\matlabtextA $\hat{t}_s^{\mathtt{thr}}[k]$}%
\psfrag{029}[cl][cl]{\matlabtextA $r_A(t_n)$}%
\psfrag{030}[tc][tc]{\matlabtextA Time (ms)}%
\psfrag{031}[bc][bc]{\matlabtextA $\#$ molecules}%
\psfrag{032}[cl][cl]{\matlabtextA $t_s[k]$}%
\psfrag{033}[cl][cl]{\matlabtextA $\bar{r}_A(t_n)$}%
\psfrag{034}[cl][cl]{\matlabtextA $r_A(t_n)$}%
\psfrag{035}[bc][bc]{\matlabtextA $\#$ molecules}%
\psfrag{036}[cl][cl]{\matlabtextA $t_s[k]$}%
\psfrag{037}[cl][cl]{\matlabtextA $\xi_B$}%
\psfrag{038}[cl][cl]{\matlabtextA $\bar{r}_B(t_n)$}%
\psfrag{039}[cl][cl]{\matlabtextA $r_B(t_n)$}%
\psfrag{040}[bc][bc]{\matlabtextA $\#$ molecules}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $0$}%
\psfrag{001}[ct][ct]{\matlabtextA $1$}%
\psfrag{002}[ct][ct]{\matlabtextA $2$}%
\psfrag{003}[ct][ct]{\matlabtextA $3$}%
\psfrag{004}[ct][ct]{\matlabtextA $4$}%
\psfrag{005}[ct][ct]{\matlabtextA $5$}%
\psfrag{009}[ct][ct]{\matlabtextA $0$}%
\psfrag{010}[ct][ct]{\matlabtextA $1$}%
\psfrag{011}[ct][ct]{\matlabtextA $2$}%
\psfrag{012}[ct][ct]{\matlabtextA $3$}%
\psfrag{013}[ct][ct]{\matlabtextA $4$}%
\psfrag{014}[ct][ct]{\matlabtextA $5$}%
\psfrag{018}[ct][ct]{\matlabtextA $0$}%
\psfrag{019}[ct][ct]{\matlabtextA $1$}%
\psfrag{020}[ct][ct]{\matlabtextA $2$}%
\psfrag{021}[ct][ct]{\matlabtextA $3$}%
\psfrag{022}[ct][ct]{\matlabtextA $4$}%
\psfrag{023}[ct][ct]{\matlabtextA $5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextA $0$}%
\psfrag{007}[rc][rc]{\matlabtextA $10$}%
\psfrag{008}[rc][rc]{\matlabtextA $20$}%
\psfrag{015}[rc][rc]{\matlabtextA $0$}%
\psfrag{016}[rc][rc]{\matlabtextA $10$}%
\psfrag{017}[rc][rc]{\matlabtextA $20$}%
\psfrag{024}[rc][rc]{\matlabtextA $0$}%
\psfrag{025}[rc][rc]{\matlabtextA $10$}%
\psfrag{026}[rc][rc]{\matlabtextA $20$}%
%
%% </ytick>

==> Fig/Concept_ML/Concept_ML.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{019}[cl][cl]{\matlabtextA $t_s[k]$}%
\psfrag{020}[cl][cl]{\matlabtextA $\hat{t}_s^{\mathtt{ML}}[k]$}%
\psfrag{021}[cl][cl]{\matlabtextA $\mathrm{ln}(\Lambda_B^{\mathtt{ML}}(t))$}%
\psfrag{022}[bc][bc]{\matlabtextA Log Likelihood}%
\psfrag{023}[tc][tc]{\matlabtextA Time (ms)}%
\psfrag{024}[cl][cl]{\matlabtextA $t_s[k]$}%
\psfrag{025}[cl][cl]{\matlabtextA $\bar{r}_B(t_n)$}%
\psfrag{026}[cl][cl]{\matlabtextA $r_B(t_n)$}%
\psfrag{027}[bc][bc]{\matlabtextA $\#$ molecules}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $0$}%
\psfrag{001}[ct][ct]{\matlabtextA $1$}%
\psfrag{002}[ct][ct]{\matlabtextA $2$}%
\psfrag{003}[ct][ct]{\matlabtextA $3$}%
\psfrag{004}[ct][ct]{\matlabtextA $4$}%
\psfrag{005}[ct][ct]{\matlabtextA $5$}%
\psfrag{010}[ct][ct]{\matlabtextA $0$}%
\psfrag{011}[ct][ct]{\matlabtextA $1$}%
\psfrag{012}[ct][ct]{\matlabtextA $2$}%
\psfrag{013}[ct][ct]{\matlabtextA $3$}%
\psfrag{014}[ct][ct]{\matlabtextA $4$}%
\psfrag{015}[ct][ct]{\matlabtextA $5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextA $-300$}%
\psfrag{007}[rc][rc]{\matlabtextA $-250$}%
\psfrag{008}[rc][rc]{\matlabtextA $-200$}%
\psfrag{009}[rc][rc]{\matlabtextA $-150$}%
\psfrag{016}[rc][rc]{\matlabtextA $0$}%
\psfrag{017}[rc][rc]{\matlabtextA $10$}%
\psfrag{018}[rc][rc]{\matlabtextA $20$}%
%
%% </ytick>

==> Fig/Concept_Peak/Concept_Peak.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{011}[cl][cl]{\matlabtextA $t_s[k]$}%
\psfrag{012}[cl][cl]{\matlabtextA $\hat{t}_s^{\mathtt{p}}[k]$}%
\psfrag{013}[cl][cl]{\matlabtextA $\bar{r}_B(t_n)$}%
\psfrag{014}[cl][cl]{\matlabtextA $r_B(t_n)$}%
\psfrag{015}[bc][bc]{\matlabtextA $\#$ molecules}%
\psfrag{016}[tc][tc]{\matlabtextA Time (ms)}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $0$}%
\psfrag{001}[ct][ct]{\matlabtextA $1$}%
\psfrag{002}[ct][ct]{\matlabtextA $2$}%
\psfrag{003}[ct][ct]{\matlabtextA $3$}%
\psfrag{004}[ct][ct]{\matlabtextA $4$}%
\psfrag{005}[ct][ct]{\matlabtextA $5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextA $0$}%
\psfrag{007}[rc][rc]{\matlabtextA $5$}%
\psfrag{008}[rc][rc]{\matlabtextA $10$}%
\psfrag{009}[rc][rc]{\matlabtextA $15$}%
\psfrag{010}[rc][rc]{\matlabtextA $20$}%
%
%% </ytick>

==> Fig/PDF_SNR10_T0406/PDF_SNR10_T0406.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{016}[cl][cl]{\matlabtextA TT Sync.}%
\psfrag{017}[cl][cl]{\matlabtextA PO Sync.}%
\psfrag{018}[cl][cl]{\matlabtextA ML Sync.}%
\psfrag{019}[bc][bc]{\matlabtextA c)}%
\psfrag{020}[bc][bc]{\matlabtextA PDF}%
\psfrag{021}[tc][tc]{\matlabtextA Normalized Synchronization Error, $\bar{e}_t[k]$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $\matlabfragNegXTick 2$}%
\psfrag{001}[ct][ct]{\matlabtextA $\matlabfragNegXTick 1.5$}%
\psfrag{002}[ct][ct]{\matlabtextA $\matlabfragNegXTick 1$}%
\psfrag{003}[ct][ct]{\matlabtextA $\matlabfragNegXTick 0.5$}%
\psfrag{004}[ct][ct]{\matlabtextA $0$}%
\psfrag{005}[ct][ct]{\matlabtextA $0.5$}%
\psfrag{006}[ct][ct]{\matlabtextA $1$}%
\psfrag{007}[ct][ct]{\matlabtextA $1.5$}%
\psfrag{008}[ct][ct]{\matlabtextA $2$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{009}[rc][rc]{\matlabtextA $10^{-4}$}%
\psfrag{010}[rc][rc]{\matlabtextA $10^{-3}$}%
\psfrag{011}[rc][rc]{\matlabtextA $10^{-2}$}%
\psfrag{012}[rc][rc]{\matlabtextA $10^{-1}$}%
\psfrag{013}[rc][rc]{\matlabtextA $10^{0}$}%
\psfrag{014}[rc][rc]{\matlabtextA $10^{1}$}%
\psfrag{015}[rc][rc]{\matlabtextA $10^{2}$}%
%
%% </ytick>

==> Fig/PDF_SNR10_T0812/PDF_SNR10_T0812.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{016}[cl][cl]{\matlabtextA TT Sync.}%
\psfrag{017}[cl][cl]{\matlabtextA PO Sync.}%
\psfrag{018}[cl][cl]{\matlabtextA ML Sync.}%
\psfrag{019}[bc][bc]{\matlabtextA a)}%
\psfrag{020}[bc][bc]{\matlabtextA PDF}%
\psfrag{021}[tc][tc]{\matlabtextA Normalized Synchronization Error, $\bar{e}_t[k]$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $\matlabfragNegXTick 2$}%
\psfrag{001}[ct][ct]{\matlabtextA $\matlabfragNegXTick 1.5$}%
\psfrag{002}[ct][ct]{\matlabtextA $\matlabfragNegXTick 1$}%
\psfrag{003}[ct][ct]{\matlabtextA $\matlabfragNegXTick 0.5$}%
\psfrag{004}[ct][ct]{\matlabtextA $0$}%
\psfrag{005}[ct][ct]{\matlabtextA $0.5$}%
\psfrag{006}[ct][ct]{\matlabtextA $1$}%
\psfrag{007}[ct][ct]{\matlabtextA $1.5$}%
\psfrag{008}[ct][ct]{\matlabtextA $2$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{009}[rc][rc]{\matlabtextA $10^{-4}$}%
\psfrag{010}[rc][rc]{\matlabtextA $10^{-3}$}%
\psfrag{011}[rc][rc]{\matlabtextA $10^{-2}$}%
\psfrag{012}[rc][rc]{\matlabtextA $10^{-1}$}%
\psfrag{013}[rc][rc]{\matlabtextA $10^{0}$}%
\psfrag{014}[rc][rc]{\matlabtextA $10^{1}$}%
\psfrag{015}[rc][rc]{\matlabtextA $10^{2}$}%
%
%% </ytick>

==> Fig/PDF_SNR5_T0812/PDF_SNR5_T0812.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{016}[cl][cl]{\matlabtextA TT Sync.}%
\psfrag{017}[cl][cl]{\matlabtextA PO Sync.}%
\psfrag{018}[cl][cl]{\matlabtextA ML Sync.}%
\psfrag{019}[bc][bc]{\matlabtextA b)}%
\psfrag{020}[bc][bc]{\matlabtextA PDF}%
\psfrag{021}[tc][tc]{\matlabtextA Normalized Synchronization Error, $\bar{e}_t[k]$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $\matlabfragNegXTick 2$}%
\psfrag{001}[ct][ct]{\matlabtextA $\matlabfragNegXTick 1.5$}%
\psfrag{002}[ct][ct]{\matlabtextA $\matlabfragNegXTick 1$}%
\psfrag{003}[ct][ct]{\matlabtextA $\matlabfragNegXTick 0.5$}%
\psfrag{004}[ct][ct]{\matlabtextA $0$}%
\psfrag{005}[ct][ct]{\matlabtextA $0.5$}%
\psfrag{006}[ct][ct]{\matlabtextA $1$}%
\psfrag{007}[ct][ct]{\matlabtextA $1.5$}%
\psfrag{008}[ct][ct]{\matlabtextA $2$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{009}[rc][rc]{\matlabtextA $10^{-4}$}%
\psfrag{010}[rc][rc]{\matlabtextA $10^{-3}$}%
\psfrag{011}[rc][rc]{\matlabtextA $10^{-2}$}%
\psfrag{012}[rc][rc]{\matlabtextA $10^{-1}$}%
\psfrag{013}[rc][rc]{\matlabtextA $10^{0}$}%
\psfrag{014}[rc][rc]{\matlabtextA $10^{1}$}%
\psfrag{015}[rc][rc]{\matlabtextA $10^{2}$}%
%
%% </ytick>
